DeepABM: Scalable, efficient and differentiable agent-based simulations via graph neural networks

We introduce DeepABM, a framework for agent-based modeling that leverages geometric message passing of graph neural networks for simulating action and interactions over large agent populations. Using DeepABM allows scaling simulations to large agent populations in real-time and running them efficiently on GPU architectures. To demonstrate the effectiveness of DeepABM, we build DeepABM-COVID simulator to provide support for various non-pharmaceutical interventions (quarantine, exposure notification, vaccination, testing) for the COVID-19 pandemic, and can scale to populations of representative size in real-time on a GPU. Specifically, DeepABM-COVID can model 200 million interactions (over 100,000 agents across 180 time-steps) in 90 seconds, and is made available online to help researchers with modeling and analysis of various interventions. We explain various components of the framework and discuss results from one research study to evaluate the impact of delaying the second dose of the COVID-19 vaccine in collaboration with clinical and public health experts. While we simulate COVID-19 spread, the ideas introduced in the paper are generic and can be easily extend to other forms of agent-based simulations. Furthermore, while beyond scope of this document, DeepABM enables inverse agent-based simulations which can be used to learn physical parameters in the (micro) simulations using gradient-based optimization with large-scale real-world (macro) data. We are optimistic that the current work can have interesting implications for bringing ABM and AI communities closer.

==> files/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Part 1 -> Need for simulations
% Successfully navigating the pandemic --> what-if questions. Likely to have a huge impact on human society in the upcoming decade. Agent-based modeling emerged as central solution: i) study action and interaction heterogenous populations, and ii) analyse emergent effects of {behavioral and clinical} interventions on the same.
The coronavirus pandemic has had significant impact of global society and economy. Successfully navigating the phase requires answering a series of 'what-if' questions which can have long lasting implications on the future of human society. Agent-based modeling (ABMs) have emerged as a central tool to help policy makers take critical decisions which may have often have non-obvious implications. In particular, ABMs are a powerful tool that enable us to i) study the action and interaction of large heterogeneous populations, and ii) analyse the emergent effects of {behavioral and clinical} interventions on the same. While ABMs are powerful descriptive tools, emergent behavior can be highly sensitive to scale of agent-populations and calibration of free-parameters. Conventional ABM frameworks such as Mesa and Net-logo follow an object oriented design. While conceptually appealing, these are often inefficient to scale to large populations. In this work, we introduce the DeepABM framework which adapts graph neural networks and 

% Part 2 -> DeepABM and scale, efficiency to ABMs
% DeepABM -- new ABM framework. Network-centric approach. Model interactions and disease spreading using message passing in graph neural networks. Massively parallelize interactions over induced sub-graphs helps improve speed.

% Part 3 -> DeepABM-COVID features and potential. Results from study
% DeepABM-COVID-19 simulations -> support for many interventions. Plots in Fig 1 and demo here. Vaccination has emerged as key tool to control viral spread and support efforts towards restoring normal life. We extensively conduct simulations to study effect of delaying 2nd dose of COVID-19 vaccine. {results in Romero et al paper}

% Part 4 -> Our contributions can be summarized as:


==> files/related_work.tex <==
\section{Related Work}
\label{sec:related-work}

==> outline2.tex <==
Title: \textit{DeepABM-COVID} for Agent-based Simulations to Evaluate COVID-19 Interventions: The Case for Delaying Second Dose Vaccines

\textit{Sec 1.} Introduction
<DeepABM {and Benefits} + COVID-Framework + Need to focus on Vaccination {Esma's introduction}>

 -- ABMs have been used commonly to analyze complex interactions and situations, and more recently have been deployed for COVID-19 analysis. 
 -- Traditionally, these ABMS use XXXX
 -- In our recent work to analyze the effectivenes soff XXXX, we developed a more efficient??? framework to build and run ABMS
 -- Traditionally, ABMS do this, while we do THAT
 -- Phase-A: [DeepABM] can model large populations {> 100k agents} with 200 million interactions over 180 time-steps in real-time as well as run on GPU. We bring machine learning ideas and developments to the ABM community.

-- Phase-B: We adapt this to design a framework for simulating covid-19 interventions with support for a) DEN b) Testing c) Vaccination d) Viral Strains. Add a couple of plots for testing and vaccination. We can implemented a plug-n-play dashboard for applying covid-19 interventions. Talk about it's features in 1-2 sentences. See demo <at link>.

[Segway] Considering relevance and urgency of problem, we specifically focus on vaccination and particular public health implications of delaying second dose of vaccines.

 -- Phase-C: in this paper, we explain several technical details of the ABM simulation framework that we built and deployed to obtain the results presented in Romera BMJ paper... 
 
 -- Explain the problem why it is important (Esma's Intro) 


\textit{Sec 2}. DeepABM-COVID Framework
    -- [DeepABM-COVID design and features]: Agent State, Infection Model + Disease Progression, Interaction Networks, Interventions.
    -- Our Implementation of the ABM:
        -> Model interaction networks as graph neural networks and disease spreading as a message passing instance over {induced} subgraphs.
        -> Fundamental assumption is that interactions within a time-step are permutation invariant which enables this.
        -> Since we can do that, we can parallelize interactions over sub-graphs and run efficiently on GPU. This gives major speed-up. For instance, \textit{in Mesa: 5 hours run-time goes to 90-sec with DeepABM}.


\textit{Sec 3.} Experiments and Results 
    -- Public Health Impact of Delaying Second Dose of COVID-19 Vaccine
        -> 
    -- Experiments and Results
        -> 


==> wsc21style.tex <==
%
%
% File contains:
%   fancyhdr.sty
%   psfig.sty
%   url.sty
%   wsc.bst
%   wscpaperproc.cls
%   wscsetup.sty
%   wsc.sty
%   wscbib.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



